Efficient Training of Self-Supervised Speech Foundation Models on a Compute Budget

Despite their impressive success, training foundation models remains computationally costly. This paper investigates how to efficiently train speech foundation models with self-supervised learning (SSL) under a limited compute budget. We examine critical factors in SSL that impact the budget, including model architecture, model size, and data size. Our goal is to make analytical steps toward understanding the training dynamics of speech foundation models. We benchmark SSL objectives in an entirely comparable setting and find that other factors contribute more significantly to the success of SSL. Our results show that slimmer model architectures outperform common small architectures under the same compute and parameter budget. We demonstrate that the size of the pre-training data remains crucial, even with data augmentation during SSL training, as performance suffers when iterating over limited data. Finally, we identify a trade-off between model size and data size, highlighting an optimal model size for a given compute budget.

==> tables/1-superb-full-table.tex <==
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|l|l}
\toprule
Downstream Tasks & Datasets & Evaluation Metrics \\
\midrule
\textbf{ASR} (Automatic Speech Recognition) & LibriSpeech~\cite{librispeech} & word error rate (WER) $\downarrow$ \\
\textbf{PR} (Phoneme Recognition) & LibriSpeech~\cite{librispeech} & phone error rate (PER) $\downarrow$ \\
\textbf{ASV} (Automatic Speaker Verification) & VoxCeleb1~\cite{voxceleb1} & equal error rate (EER) $\downarrow$ \\
\textbf{SD} (Speaker Diarization) & LibriMix~\cite{librimix} & diarization error rate (DER) $\downarrow$ \\
\textbf{SF} (Slot Filling) & Audio SNIPS~\cite{snips} & slot value CER $\downarrow$ / slot-type F1 score $\uparrow$ \\
\textbf{KS} (Keyword Spotting) & Speech Commands v1.0~\cite{speech_commands} & accuracy (ACC) $\uparrow$ \\
\textbf{IC} (Intent Classification) & Fluent Speech Commands~\cite{fluent_commands} & accuracy (ACC) $\uparrow$ \\
\textbf{SID} (Speaker Identification) & VoxCeleb1~\cite{voxceleb1} & accuracy (ACC) $\uparrow$ \\
\textbf{ER} (Emotion Recognition) & IEMOCAP~\cite{iemocap} & accuracy (ACC) $\uparrow$ \\
\bottomrule
\end{tabular}
\caption{
SUPERB downstream tasks used in our experiments.
The symbol $\downarrow$ indicates the goal of obtaining a lower score in the metric, whereas the symbol $\uparrow$ signifies the aim of achieving a higher score in the metric.}
% \vspace{-3mm}
\label{table:superb}
\end{table*}
